Revisiting Graph Contrastive Learning from the Perspective of Graph Spectrum

Graph Contrastive Learning (GCL), learning the node representations by augmenting graphs, has attracted considerable attentions. Despite the proliferation of various graph augmentation strategies, some fundamental questions still remain unclear: what information is essentially encoded into the learned representations by GCL? Are there some general graph augmentation rules behind different augmentations? If so, what are they and what insights can they bring? In this paper, we answer these questions by establishing the connection between GCL and graph spectrum. By an experimental investigation in spectral domain, we firstly find the General grAph augMEntation (GAME) rule for GCL, i.e., the difference of the high-frequency parts between two augmented graphs should be larger than that of low-frequency parts. This rule reveals the fundamental principle to revisit the current graph augmentations and design new effective graph augmentations. Then we theoretically prove that GCL is able to learn the invariance information by contrastive invariance theorem, together with our GAME rule, for the first time, we uncover that the learned representations by GCL essentially encode the low-frequency information, which explains why GCL works. Guided by this rule, we propose a spectral graph contrastive learning module (SpCo), which is a general and GCL-friendly plug-in. We combine it with different existing GCL models, and extensive experiments well demonstrate that it can further improve the performances of a wide variety of different GCL methods.

==> sec/sec_model_.tex <==
\section{Spectral Graph Contrastive Learning}
\subsection{Theoretical derivation and formulation of SpCo}
\label{derivation}
In this section, we tempt to learn an augmented graph from original graph based on the GAME rule. Based on eigenvalue perturbation formula~\eqref{pertu} removing the high-order term $\mathcal{O}(||\Delta\bm{A}||)$, we have:
\begin{subequations}
\begin{align} 
\Delta \lambda_i& \approx \bm{u}_i^\top\Delta\bm{A}\bm{u}_i-\lambda_i\bm{u}_i^\top\Delta\bm{D}\bm{u}_i \notag\\
& = \sum_{m,n} [(\bm{u}_i\bm{u}_i^\top)*\Delta \bm{A}]_{m,n} - \lambda_i \bm{u}_i^\top\Delta \bm{D} \bm{u}_i \label{b}\\
& = <\bm{S}_i, \Delta \bm{A}> - \lambda_i \bm{u}_i^\top\Delta \bm{D} \bm{u}_i. \label{c}
\end{align}
\end{subequations}
In eq.~\eqref{b}, we use '*' to represent element-wise product, and use $<\bm{P}, \bm{Q}>$ to represent the sum of all elements of $\bm{P} * \bm{Q}$ in eq.~\eqref{c}. Before further derivation, we give a lemma as following:
\begin{Lemma}
\label{lemma}
$|\lambda_i\bm{u}_i^\top\Delta\ \bm{D}\bm{u}_i|\ \leq N|\lambda_i|$.
\end{Lemma}
This lemma is proved in Appendix~\ref{proof_lemma}. Then with Lemma~\ref{lemma}, we gather the changes of all eigenvalues together, and have the following two theorems:
\begin{Theorem}
Given $\Delta_{total} =\sum_i \alpha_i|\Delta \lambda_i|$, we have
\label{lllalla}
\begin{align*}
\Delta_{total} \iff \sum_i \alpha_i\left|<\bm{S}_i, \Delta \bm{A}>\right|\geq \sum_i\alpha_i\left|<\bm{S}_i, \Delta_{\bm{A+}}>\right|-\sum_j a_j\left|<\bm{S_j}, \Delta_{\bm{A-}}>\right|=\Delta_+-\Delta_-,
\end{align*}
where $\alpha_i\geq 0$ is the weight for the change of $\lambda_i$. Formally, we have $\Delta\bm{A}=\Delta_{\bm{A+}}-\Delta_{\bm{A-}}$, where $\Delta_{\bm{A+}}$ and $\Delta_{\bm{A-}}$ indicate which edge is added and deleted, respectively. 
\end{Theorem}
% The proof is in Appendix~\ref{proof_2}. From this theorem, we can control the similarity between $\Delta \bm{A}$ and $\bm{S}_i$ to adjust the size of $\left|\Delta \lambda_i\right|$. Our purpose is to make the changes of eigenvalues meet the GAME rule, where $|\Delta \lambda_i|$ in $\mathcal{F_L}$ is smaller than that in $\mathcal{F_H}$. Actually, we can achieve this target by maximizing the $\Delta_{total}$, and the following theorem guarantees correctness of this operation:
\begin{Theorem}
\label{close}
Given N eigenspaces $\left[\bm{S_1},\dots,\bm{S_N}\right]$, if $|<\bm{S}_i,\Delta \bm{A}>|$ is maximized, then $\forall j,\ |<\bm{S_j},\ \Delta \bm{A}>| \to 0$.
\end{Theorem}
The proof is given in Appendix~\ref{proof_2} and~\ref{proof_3}. Theorem~\ref{close} implies that $\Delta \bm{A}$ can only be related to one of these eigenspaces. Please recall that we need $|\Delta \lambda_i|$ in $\mathcal{F_L}$ is smaller than that in $\mathcal{F_H}$. Therefore, we first make $\alpha_i$ is larger for $\Delta \lambda_i$ in $\mathcal{F_H}$ than in $\mathcal{F_L}$. Then, we maximize $\Delta_{total}$, and $\Delta \bm{A}$ will only be related to $\bm{S}_i$ in $\mathcal{F_H}$. That means $|\Delta \lambda_i|$ in $\mathcal{F_H}$ will be larger. Particularly, Theorem~\ref{lllalla} indicates that we can maximize $\Delta_+$ and minimize $\Delta_-$ simultaneously to maximize $\Delta_{total}$. For $\Delta_+$, we can maximize it by following formula:
\begin{subequations}
\begin{align} 
\Delta_+ &=\sum_i \alpha_i\left|<\bm{S}_i, \Delta_{\bm{A+}}>\right| = |\sum_i \alpha_i<\bm{S}_i, \Delta_{\bm{A+}}>|  \notag\\
&=|<\sum_i\alpha_i\bm{u}_i\bm{u}_i^\top,\ \Delta_{\bm{A+}}>| =\left|<\bm{U}g(\lambda)\bm{U}^\top, \ \Delta_{\bm{A+}}>\right|=\left|<\bm{\mathcal{C}}, \ \Delta_{\bm{A+}}>\right|.  \label{bb}
\end{align}
\end{subequations}
In eq.~\eqref{bb}, we define $\bm{\mathcal{C}}=\bm{U}g(\lambda)\bm{U}^\top$ and $\alpha_i=g(\lambda_i)$, where $g(\lambda)$ should be a monotone increasing function. As can be seen, if $\Delta_{\bm{A+}}$ is learnt to be closed to some predefined $\bm{\mathcal{C}}$, $\Delta_+$ will increase.

\textbf{Setting $\bm{\mathcal{C}}$} We notice that the graph spectrum of Laplacian $\bm{\mathcal{L}}$ does meet our need about $g(\lambda)$. Therefore, we simply set $\bm{\mathcal{C}}=\Theta\bm{\mathcal{L}}$, where $\Theta$ is a parameter. We can increase $\Theta$ in a curricular way:
\begin{equation}
    \Theta = \frac{t}{T}\cdot \Theta',
    \label{uupp}
\end{equation}
where $\Theta'$ is a constant, and $\Theta$ is used in $t$th epoch. $T$ is the total epoch.

With eq.~\eqref{bb}, we give the following optimization objective:
% So far, we have got a target to guide the learning of $\Delta_{\bm{A+}}$ that maximizes $\left|<\bm{\mathcal{C}}, \ \Delta_{\bm{A+}}>\right|$ to maximize $\Delta_+$ and then $\Delta_{total}$. In addition, we consider two extra conditions to make $\Delta_{\bm{A+}}$ more reasonable. Firstly, we do not want edges in $\Delta_{\bm{A+}}$ only exist in some fixed pairs of nodes, which definitely constrains the capacity of $\Delta_{\bm{A+}}$. On the contrary, we prefer that $\Delta_{\bm{A+}}$ should be a denser matrix, where more edges are exposed to be optimized to boost the results. Secondly, $\Delta_{\bm{A+}}$ should not be optimized arbitrarily without any constraints. That's to say, the row sum and column sum of $\Delta_{\bm{A+}}$ should be accord with some special distribution. Combined with the above conditions, we give a more comprehensive and complete target for $\Delta_{\bm{A+}}$ as following:
\begin{equation}
    \label{target}
    \mathcal{J} = <\bm{\mathcal{C}}, \ \Delta_{\bm{A+}}>^2+  \epsilon H(\Delta_{\bm{A+}})+<\bm{f},\Delta_{\bm{A+}}\mathbbm{1}_n-\bm{a}>+<\bm{g},\Delta_{\bm{A+}}^\top\mathbbm{1}_n-\bm{b}>,
\end{equation}
where $H(\bm{P})$ is the entropy regularization, defined as $-\sum_{i, j}\bm{P}_{i, j}(\log(\bm{P}_{i, j})-1)$ \citep{ot}, and $\epsilon$ is the weight of this term. This term exposes more edges in $\Delta_{\bm{A+}}$ to optimization. The last two terms are Lagrange constraint conditions, where $\bm{f}\in \mathbb{R}^{N}$ and $\bm{g}\in \mathbb{R}^{N}$ are Lagrange multipliers, and $\bm{a}\in \mathbb{R}^{N\times 1}$ and $\bm{b}\in \mathbb{R}^{N\times 1}$ are distributions\footnote{We define $\bm{a}$ and $\bm{b}$ are both node degree distribution in this paper.} that the row and column sums of $\Delta_{\bm{A+}}$ should meet. Next, the partial of $\mathcal{J}$ with respect to $\Delta_{\bm{A+}}$ is as following:
\begin{subequations}
\begin{align} 
\partial \mathcal{J}\ /\ \partial (\Delta_{\bm{A+}})_{ij}&=2<\bm{\mathcal{C}}, \ \Delta_{\bm{A+}}>\bm{\mathcal{C}}_{ij}-\epsilon \log (\Delta_{\bm{A+}})_{ij} + \bm{f}_i+\bm{g}_j  \label{aaa}\\
&=m_{ij}+2\bm{\mathcal{C}}_{ij}^2(\Delta_{\bm{A+}})_{ij}-\epsilon \log (\Delta_{\bm{A+}})_{ij}+\bm{f}_i+\bm{g}_j, \label{bbb}
\end{align}
\end{subequations}
where we separate $2\bm{\mathcal{C}}_{ij}^2(\Delta_{\bm{A+}})_{ij}$ from $2<\bm{\mathcal{C}}, \ \Delta_{\bm{A+}}>\bm{\mathcal{C}}_{ij}$, and set the rest part as $m_{ij}$. The next theorem points out when $\mathcal{J}$ can get the maximal value in the domain of definition $(\Delta_{\bm{A+}})_{ij}\in(0, 1)$:
\begin{Theorem}
\label{theorem 4}
Given\ $(\Delta_{\textbf{A+}})_{ij}\in(0,1)$,\ $\mathcal{J}$\ exists\ the\ maximal\ value,\ iff\\
(1) $\bm{\mathcal{C}}_{ij}^2 < -\frac{\bm{f}_i+\bm{g}_j+m_{ij}}{2}$,\text{ and}\ $\bm{f}_i+\bm{g}_j+m_{ij}<0$,\ or\\
(2) $\frac{\epsilon}{2}<\bm{\mathcal{C}}_{ij}^2<\frac{\epsilon}{2}\exp(-\frac{\bm{f}_i+\bm{g}_j+m_{ij}+\epsilon}{2})$,\text{ and}\ $\bm{f}_i+\bm{g}_j+m_{ij}+\epsilon<0$.
\end{Theorem}
We provide the proof in the Appendix~\ref{proof_4}. Normally, we should let eq.~\eqref{bbb} equal to zero and get the analytical solution of $(\Delta_{\bm{A+}})_{ij}$. However, eq.~\eqref{bbb} is a transcendental equation because of the existence of linear term and logarithm. 
Thus, we require eq.~\eqref{aaa} to equal to 0. Specifically, in each training epoch, we firstly calculate "$<\bm{\mathcal{C}}, \Delta_{\bm{A+}}>$", where $\Delta_{\bm{A+}}$ is replaced by $\Delta_{\bm{A+}}'$ got from the last epoch. So, the first term in eq.~\eqref{aaa} is a constant, and the matrix form of solution of current epoch is:
\begin{equation}
\label{solution}
    \Delta_{\bm{A+}} = diag(\bm{u})\exp\left(2<\bm{\mathcal{C}}, \Delta_{\bm{A+}}'>\bm{\mathcal{C}}\ /\ \epsilon\right)diag(\bm{v})=\bm{U_{+}K_{+}V_{+}},
\end{equation}
where $\bm{u}_i=\exp\big(\frac{\bm{f}_i}{\epsilon}\big)$ and $\bm{v}_j=\exp\big(\frac{\bm{g}_j}{\epsilon}\big)$. Please note that we require the $\Delta_{\bm{A+}}$ must meet the Lagrange constraint conditions, mentioned in eq.~\eqref{target}. So, we have the requirements: $\bm{u}*\left(\bm{K_{+}v}\right)=\bm{a}$ and $ \bm{v}*\left(\bm{K_{+}}^\top \bm{u}\right)=\bm{b}$. We solve this matrix scaling problem \citep{nemirovski1999complexity} by iteratively updating $\bm{u}$ and $\bm{v}$:
\begin{equation}
    \bm{u}^{({l}+1)}=\bm{a}\ /\ \left(\bm{K_{+}v}^{(l)}\right) \quad \text{and} \quad \bm{v}^{({l}+1)}=\bm{b}\ /\ \left(\bm{K_{+}}^\top \bm{u}^{(l+1)}\right),
\end{equation}
where $l$ is the $l$th iteration. This process is Sinkhorn's Iteration \citep{sinkhorn}, which is given in Algorithm~\ref{Sinkhorn's Iteration Process}, referring to \citep{cuturi2013sinkhorn}. After this, the new calculated $\Delta_{\bm{A+}}$ will be used in eq.~\eqref{solution} as $\Delta_{\bm{A+}}'$ in the next training epoch. There exists a upper bound of the difference between $\Delta_{\bm{A+}}$ and $\Delta_{\bm{A+}}'$:
%We next prove a upper bound of the difference between $\Delta_{\bm{A+}}$ and $\Delta_{\bm{A+}}'$, which guarantees that the used trick does not make the solution diverge:
\begin{Theorem}
\label{theorem 5}
After Sinkhorn's Iteration, the bound between $\Delta_{\bm{A+}}$ and $\Delta_{\bm{A+}}'$ is: \\
\centerline{$\left|\alpha(\Delta_{\bm{A+}})_{ij}-(\Delta_{\bm{A+}})_{ij}'\right|\leq\frac{\alpha}{\epsilon^2(1-\gamma)}\{d(r^{(0)},\bm{a})+d(c^{(0)},\bm{b})\}+\alpha(1+\frac{|m_{ij}|}{\epsilon})$,} \\
where $\alpha=\frac{\epsilon}{2\bm{\mathcal{C}}_{ij}^2}$. $\forall (x, x')\in(\mathbb{R}^n_{+})^2$, $d(x, x')$ is the Hilbert’s projective metric \citep{bushell1973hilbert} on $\mathbb{R}^n_{+}$. $\gamma$ is $\kappa({\bm{K_{+}}})$, and $\kappa$ is contraction ratio \citep{franklin1989scaling}. $r^{(0)}$ and $c^{(0)}$ are the row and column sum vectors of $\bm{K_{+}}$.
\end{Theorem}
The proof is given in Appendix~\ref{proof_5}. The calculation of $\Delta_{\bm{A-}}$ is similar as $\Delta_{\bm{A+}}$ shown as follows: $\Delta_{\bm{A-}} = diag(\bm{u}')\exp\left(-2<\bm{\mathcal{C}}, \Delta_{\bm{A-}}'>\bm{\mathcal{C}}\ /\ \epsilon\right)diag(\bm{v}')=\bm{U_{-}K_{-}V_{-}}$. Now we can obtain $\Delta_{\bm{A+}}$ and $\Delta_{\bm{A-}}$, and $\Delta_{\bm{A}}=\Delta_{\bm{A+}}-\Delta_{\bm{A-}}$. Next, we show that the $\Delta_{\bm{A}}$ is a general component, which can be easily plugged into the current GCL to further improve them.

\subsection{Instantiation of SpCo with existing GCL}
\begin{wrapfigure}[12]{r}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.19]{fig/spco.png}
    \caption{Combine SpCo with existing GCL.}\label{spco}
\end{wrapfigure}
 As shown in Fig.~\ref{spco}, we first transform $\bm{A}$ into an augmented graph $\bm{A\_}$ as follows:
\begin{equation}
\begin{aligned}
\label{ete}
    \bm{A\_} = \bm{A}+\eta\cdot\mathbb{S}*\Delta_{\bm{A}},
\end{aligned}
\end{equation}
where $\eta$ is the combination coefficient. To make $\Delta_{\bm{A}}$ sparse, we only keep the values in a limited scope $\mathbb{S}$, for example the one-hop neighbors for each node. 
%In this equation, we know that $\bm{A}$ and $\bm{A\_}$ satisfy the GAME rule, because $\Delta_{\bm{A}}$ in $\mathcal{F_L}$ is smaller than in $\mathcal{F_H}$.
Then, we augment $\bm{A}$ and $\bm{A\_}$ with the same strategies of target GCL model $\Phi$ to generate $\bm{V_1}$ and $\bm{V_2}$. Next, $\bm{V_1}$ and $\bm{V_2}$ are used for GCL. The whole algorithm is given in Algorithm~\ref{The proposed SpCo}.

==> sec/sec_rel.tex <==
\section{Related Work}
\textbf{Graph Neural Networks.}
Recently, Graph Neural Networks (GNNs) have attracted considerable attentions, which can be broadly divided into two categories, spectral-based and spatial-based. Spectral-based GNNs are inheritance of graph signal processing, and define graph convolution operation in spectral domain. For example, \cite{spe1} utilizes Fourier bias to decompose graph signals; \cite{spe2} employs the Chebyshev expansion of the graph Laplacian to improve the efficiency. For another line, spatial-based GNNs greatly simplify above convolution by only focusing on neighbors. For example, GCN \cite{gcn} simply averages information of one-hop neighbors. GraphSAGE \cite{graphsage} only randomly fuses a part of neighbors with various poolings. GAT \cite{gat} assigns different weights to different neighbors. More detailed surveys can be found in \cite{wu2021comprehensive}.

\textbf{Graph Contrastive Learning.}
Graph Contrastive Learning has shown its distinguished capacity in unsupervised setting, and many studies have been proposed. In this paper, we mainly focus on the various augmentation strategies. Specifically, DGI \citep{dgi} contrasts between local node embedding and global summary vector. MVGRL \citep{mvgrl} proposes several strategies based on diffusion or  distance matrix. For \{GRACE \citep{grace}, GCA \citep{gca}, GraphCL \citep{graphcl}, CCA-SSG \citep{cca}\}, they can roughly be gathered into the same category: the random edge and node perturbation. There are some frameworks aiming to learn an adaptive augmentation with the help of different principles, such as AD-GCL \citep{adgcl}, InfoGCL \citep{infogcl}, DGCL \citep{dgcl} and GASSL \cite{yang2021graph}. But these studies mainly focus on graph classification task. Besides, we also notice that some papers propose augmentation free \citep{lee2021augmentation}.
